Reinforcement Learning for Omega-Regular Specifications on Continuous-Time MDP

Continuous-time Markov decision processes (CTMDPs) are canonical models to express sequential decision-making under dense-time and stochastic environments. When the stochastic evolution of the environment is only available via sampling, model-free reinforcement learning (RL) is the algorithm-of-choice to compute optimal decision sequence. RL, on the other hand, requires the learning objective to be encoded as scalar reward signals. Since doing such translations manually is both tedious and error-prone, a number of techniques have been proposed to translate high-level objectives (expressed in logic or automata formalism) to scalar rewards for discrete-time Markov decision processes (MDPs). Unfortunately, no automatic translation exists for CTMDPs. We consider CTMDP environments against the learning objectives expressed as omega-regular languages. Omega-regular languages generalize regular languages to infinite-horizon specifications and can express properties given in popular linear-time logic LTL. To accommodate the dense-time nature of CTMDPs, we consider two different semantics of omega-regular objectives: 1) satisfaction semantics where the goal of the learner is to maximize the probability of spending positive time in the good states, and 2) expectation semantics where the goal of the learner is to optimize the long-run expected average time spent in the ``good states" of the automaton. We present an approach enabling correct translation to scalar reward signals that can be readily used by off-the-shelf RL algorithms for CTMDPs. We demonstrate the effectiveness of the proposed algorithms by evaluating it on some popular CTMDP benchmarks with omega-regular objectives.

==> GFM.tex <==

Given an MDP $\Mm$ and an $\omega$-regular objective $\varphi$ given as
an $\omega$-automaton $\Aa_\varphi = (\Sigma,Q,q_0,\delta,F)$,
we want to compute an optimal strategy satisfying the
objective.
We define the satisfaction probability of $\sigma$ from starting state
$s$ as: 
\begin{equation*}
\PSemSat^\Mm_{\Aa}(s, \sigma) 
%\Pr^\Mm_\sigma(s \models \varphi)
=   \Pr{}^\Mm_\sigma(s) \set{ r \in \Runs_\sigma^\Mm(s) \colon
  L(r) \in \Ll(\Aa) }.
\end{equation*}
The optimal satisfaction probability
$\PSemSat^\Mm_{\Aa}(s)$ for specification $\Aa$ %$\Pr^\Mm_*(s\models \varphi)$
is defined as $\sup_{\sigma \in \Strat_\Mm} \Pr^\Mm_\sigma(s, \sigma)$ and we say
that $\sigma \in \Strat_\Mm$ is an optimal strategy for $\Aa$ if
$\PSemSat^\Mm_{\Aa}(s, \sigma) (s) = \PSemSat^\Mm_{\Aa}(s)$.

Given an MDP
%$\Mm = \langle S, s_0, A, T, \Sigma, L \rangle$
$\Mm = ( S, s_0, A, T, AP, L )$
and automaton
%$\mathcal{A} = \langle \Sigma, Q, q_0, \Delta, F \rangle$,
$\mathcal{A} = (2^{AP}, Q, q_0, \delta, F )$,
the
\emph{product}
%$\Mm \times \mathcal{A} = \langle S \times Q, (s_0,q_0), A \times Q,T^\times, F^\times \rangle$
$\Mm \times \mathcal{A} = ( S \times Q, (s_0,q_0), A \times Q, T^\times, F^\times )$
is an MDP with initial
state $(s_0,q_0)$
and accepting transitions $F^\times$ where
%The function
$T^\times : (S \times Q) \times (A \times Q) \pto \DIST(S \times Q)$
is defined by
\begin{multline*}
T^\times((s,q),(a,q'))(({s}',{q}')) {=}
\begin{cases}
T(s,a)({s}') & \text{if } (q,L(s,a,{s}'),{q}') {\in} \delta \\
0 & \text{otherwise.}
\end{cases}
\end{multline*}
The final state
$F^\times \subseteq (S \times Q) \times (A \times Q) \times (S
\times Q)$ is defined by $((s,q),(a,q'),(s',q')) \in F^\times$
if, and only if, $(q,L(s,a,s'),q') \in F$ and $T(s,a)(s') > 0$.
A strategy $\sigma^\times$ on the product defines a strategy $\sigma$ on the
MDP with the same value, and vice versa.  Note that for a stationary
$\sigma^\times$, the strategy $\sigma$ may need memory.
End-components and runs of the product MDP are defined just like for MDPs.

A run of $\Mm \times \mathcal{A}$ is accepting if
$\inf(r) \cap F^\times \neq \emptyset$.
We define the
\emph{syntactic satisfaction}
probabilities $\PSat^\Mm_{\Aa}((s,q), \sigma^\times)$ as the probability of
accepting runs, i.e.
\[
\Pr{}^{\Mm\times\Aa}_{\sigma^\times}(s,q) \Set{ r \in
\Runs_{\sigma^\times}^{\Mm\times\Aa}(s,q) : \inf(r) \cap F^\times
\neq \emptyset }
\]
Similarly, we define $\PSat^\Mm_{\Aa}(s)$ as the optimal probability over the
product, i.e.  $\sup_{\sigma^\times}\big(\PSat^\Mm_{\Aa}((s,q_0),
\sigma^\times)\big)$.
For a deterministic $\Aa$ the equality $\PSat^\Mm_{\Aa}(s) = \PSemSat^\Mm_{\Aa}(s)$ holds; however it is not guaranteed for nondeterministic
B\"uchi automata as the optimal resolution of nondeterministic
choices may require access to future events.
This motivates for the definition of a good-for-MDP nondeterminisitc B\"uchi automata.
A B\"uchi automaton $\Aa$ is \emph{good for MDPs} (GFM),
if $\PSat^\Mm_{\Aa}(s_0) = \PSemSat^\Mm_{\Aa}(s_0)$ holds for all
MDPs $\Mm$ and starting states $s_0$ \cite{Hahn20}.
Note that every $\omega$-regular objective can be expressed as a GFM automaton \cite{Hahn20}.
A popular class of GFM automata is suitable limit-deterministic B\"uchi automata~\cite{Hahn2015LazyPM,sickert2016limit}.
This paper considers only GFM B\"uchi automata.

The satisfaction of an $\omega$-regular objective given as a GFM automaton $\Aa$
by an MDP $\Mm$ can be formulated in terms of the accepting maximal
end-components of the product $\Mm {\times} \mathcal{A}$, i.e. the maximal
end-component that contains an accepting transition from $\F^\times$.  
The optimal satisfaction probabilities and strategies can be computed by
computing the accepting maximal end-component of $\Mm\times \Aa$ and then
maximizing the probability to reach states in such components.
The optimal strategies are positional on $\Mm\times\Aa$ and characterize a finite memory strategy over $\Mm$ maximizing satisfaction probability of the learning objective given by $\Aa$.


==> MarsRoverExample.tex <==
Following example gives an intuition on satisfaction and expectation semantics.
\begin{example}[Satisfaction or Expectation?]
The grid-world shown in Figure~\ref{fig:grid-world} (adapted from \cite{HahnPSSTW19}) represents four zones (represented by $s_0$ to $s_3$ in the figure) on the Mars surface. 
Suppose that a mission to Mars arrives in Zone~$0$ (a known, safe territory) and is expected to explore the terrain in a safe fashion, gather and transmit information, and stay alive to maximize the return on the mission.
For simplicity, assume that Zone $1$ (purple) models a crevasse harmful to the safe operations, while zones $2$ and $3$ are central to exploration mission and are analogous in their information contents.

\input{automata_drawing}
Given the unknown uncertainty of the terrain of Mars, the system is modeled as a CTMDP with associated uncertainty on the time of various actions where the exit rate of action $a$ from Zone (state) $0$ is denoted by $\lambda(0,a)$. In other words, when selected an action $a$ in a state $s$, the probability of spending $t$ time units in $s$ before taking $a$ is given by the cumulative distribution function $1 - e^{- \lambda(0,a)t}$.
Assume that the action $b$ from Zone $0$ goes to Zone $2$ with rate $r$ (high probability) and to Zone $1$ with rate  $(\lambda(0,b) - r)$ (low probability).
% \textcolor{red}{there is an action $b$ and a label for state $b$, this would create confusion.}
The mission objective is to avoid Zone $1$ (blue zone) while infinitely often visiting the Zone $2$ or $3$ (the green zones). 
It can be captured in LTL~\cite{Baier08} as:
\[
\varphi = (\always \neg \mathtt{p}) \wedge (\always(\eventually \mathtt{g}))
\]
specifying that across the infinite horizon {\bf globally} (i.e. at every step expressed as temporal modality, $\always$) avoid the blue region ($\neg b$), and globally {\bf finally} (i.e. at some time in the future expressed as temporal modality, $\eventually$) reach the green region, i.e. $(\always (\eventually g))$. 
The $GF \phi$ modality is often referred as \emph{infinitely often $\phi$}.
LTL combines these temporal operators using the standard propositional logic connectives such as: and ($\wedge$), or ($\lor$), not ($\neg$), and implication ($\to$).

This declarative specification can also be expressed using the B\"uchi automaton shown in Figure~\ref{fig:grid-world} (center) where the double circled states (here, $q_1$) denote accepting states.
The B\"uchi automata can be used as the monitors of the behaviors of the learner over the environments given as CTMDPs. For our example, it is visualized by taking the synchronous product (an extended space CTMDP) of the CTMDP with the automaton shown in Figure~\ref{fig:grid-world} (right).

For the satisfaction semantics on the product CTMDP, our goal is to maximize the probability that every infinite horizon behavior visits the accepting state infinitely often, while for the expectation semantics the goal is to maximize the expected time the system dwells in the accepting state.
\begin{itemize}
    \item \noindent {\bf Satisfaction Objective.} 
Consider the case where we have one Mars rover in this mission. Hence, our goal naturally is to maximize the probability of visiting green zones infinitely often while avoiding the blue zone (the satisfaction semantics).
In this case, the optimal schedule is to choose actions $a$ and $c$ indefinitely, i.e. the schedule $(a \to c)^\omega$, that satisfies the objective with probability $1$.
Note that it does not make sense to choose action $b$ no matter how low the probability is to reach the blue zone.
\item 
\noindent {\bf Expectation Objective.} Consider an alternative setting where we have a fleet of drones (we are okay in losing some drones as long as we maximize the mission objective) that needs to be sent to the surveillance of zone $2$ or $3$. 
Suppose that due to unforeseeable circumstances the mission may cease operation any time, and hence the goal is to maximize total expected time spent in the green zones ($2$ and $3$).
The schedule $(a\to c)^\omega$ is not optimal anymore as it may dwell a considerable amount in the Zone $0$. 
On the hand hand any drone that chooses $b$ in Zone $0$ risks moving to Zone $1$ with a small probability.
As our goal is to maximize the expected time over a large group of drones, the expectation semantics captures this intent and the optimal schedule is to start with action $b$.
\end{itemize}
\end{example}

==> RL_methods.tex <==
% Popular model-free reinforcement learning algorithms like TD($\lambda$) and Q-learning for CTMDPs were defined by Bradtke and Duff in \cite{BD94}. We give a small summary of these methods for the reader.
% \subsection{Value functions for states}
% An optimal policy for a discounted objective is obtained by defining expected discounted reward for each state. These are called `value' of a state. The value of a state $s$ in CTMDP $\Mdp$ under a pure strategy $\sigma$ is denoted by $\valuef$. The expected reward from a transition from state $s$ to $s'$ on action $a$ is defined as \begin{equation*}
% \begin{split}
%   \erew(s,s',a) & = rew(s,a) +\\
%   & \int_{0}^{\infty} \int_{0}^{t} e^{\lambda(s,a)x}rew(s)dx dF(t|s,a)  
% \end{split}
%  \end{equation*}
% The expected discount factor on value of $s'$ in the transition from $s$ to $s'$ on action $a$ is defined as \\
% $\gamma = \int_{0}^{\infty} e^{\lambda(s,a)t}dF(t|s,a)$\\
% Now we can define $\valuef$ as 
% \begin{equation}
%     \begin{split}
%         \valuef & = \sum_{s'\in \states} \Delta(s,\sigma(s),s').\erew(s,s',\sigma(s)) + \\
%         & \gamma \sum_{s' \in \states} \Delta(s,\sigma(s),s') v_{\sigma}(s')
%     \end{split}
% \end{equation}
% \subsection{Temporal difference learning}
% In MDPs, TD(0) algorithm stores value for each state of the MDP. When a reward $r(s,s',a)$ is observed from a transition from $s$ to $s'$ on an action $a$, the value function is updated. If current value of $s$ is denoted by $\kvalue$, then the new value is given by \\
% $$\newvalue = \kvalue + \alpha_{k}[r(s,s',a) + \gamma v^{(k)}(s') - \kvalue]$$\\
% where $\alpha_{k}$ is the learning rate. It is proven that for a suitable $\alpha$, the TD(0) algorithm converges to the real value of the state with probability 1. \\ 
% The algorithm is similar for CTMDPs where the only difference is in the computation of the value function. The value function is intended to solve equation (1). 
% \begin{equation}
% \begin{split}
% \newvalue = \kvalue + \alpha_{k}[r(s,a) + \frac{1 - e^{-\lambda(s,a)\tau}}{\lambda(s,a)}r(s) + \\ e^{\lambda(s,a)\tau}v^{(k)}(s') - v^{(k)}(s)]    
% \end{split}
% \end{equation}
% where the sampled transition time from $s$ to $s'$ is $\tau$, $r(s,a) + \frac{1 - e^{-\lambda(s,a)\tau}}{\lambda(s,a)}r(s)$ is the sample reward from the transition and $e^{\lambda(s,a)\tau}$ is the sample discount on the value of the next state $s'$. TD($\lambda$) learning rule can be defined from this equation.

% \subsection{Q-learning}
% Q-learning is a model-free reinforcement learning algorithm which is similar to TD(0). For an MDP $\Mdp$ and a strategy $\sigma$ we define a function $\valueq(s,a)$ for each state $s$ and action $a$. The Q-function must satisfy the following equation 
% \begin{equation}
%     \begin{split}
%         \valueq(s,a) = rew(s,s',a) + \gamma \sum_{s' \in \states} P(s,s',a)\valueq(s',\sigma(s'))
%     \end{split}
% \end{equation}
% Here, the main difference is that $a$ can be any action and not necessarily the action chosen by $\sigma$. Therefore, $\valueq(s,a)$ gives the expected discounted reward from choosing an action $a$ in state $s$ under a policy $\sigma$. The optimal Q-function is denoted by $\optvalueq$. The optimal Q-function $\optvalueq$ satisfies the Bellman-style optimality equation 
% \begin{equation}
%     \begin{split}
%         \optvalueq(s,a) = r(s,s',a) + \gamma \sum_{s' \in \states} p(s,s',a) \max_{a' \in \actions} \optvalueq(s',a')
%     \end{split}
% \end{equation}
% Q-learning uses stochastic approximation to iteratively refine the $\optvalueq$ function. When a transition from state $s$ to $s'$ on action $a$ is observed, the $\optvalueq$ function is updated according to the following learning rule
% \begin{equation}
% \begin{split}
%     \newvaluef(s,a) &= \kvaluef(s,a) + [r(s,s',a) +\\& \gamma \cdot \max_{a'} \kvaluef(s',a') - \kvalue]
% \end{split}    
% \end{equation}
% We can define a similar learning rule for CTMDPs. The optimal Q-function for a CTMDP satisfies the following equation 
% \begin{equation}
%     \begin{split}
%         \optvalueq(s,a) = \sum_{s' \in \states} \Delta(s,a,s') \erew(s,s',a) + \\
%         \gamma \sum_{s'\in \states} \Delta(s,a,s') \max_{a' \in \actions} \valueq(s',a')
%     \end{split}
% \end{equation}
% This leads to the following Q-learning rule for CTMDPs 
% \begin{equation}
%     \begin{split}
%         \newvaluef(s,a) = \kvaluef(s,a) + \alpha_{k}[rew(s,a)d + \frac{1-e^{-\lambda(s,a)\tau}}{\lambda(s,a)}r(s) + \\
%         e^{-\lambda(s,a)\tau} \max_{a'} \kvaluef(s',a') - \kvaluef(s,a)]
%     \end{split}
% \end{equation}
% % From the above equations it is clear that Q-learning and TD(0) works in a similar fashion. \*       
        


==> algorithms.tex <==
\begin{algorithm}
\caption{Algorithm for satisfaction semantics}\label{algo:sat}
\hspace*{\algorithmicindent} \textbf{Input:}  \text{Initial state $s_{init}$, SLDBW $A$, discount factor $\gamma$,}\\
\hspace*{\algorithmicindent} \hspace{11mm}\text{reward function $R'$, number of episodes $k$,} \\
\hspace*{\algorithmicindent}\hspace{11mm} \text{learning rate $\alpha$}\\
\hspace*{\algorithmicindent} \textbf{Output:}  \text{$Q_f$}
\begin{algorithmic}[1]
\STATE Initialise $Q_f$ to all zeroes
\STATE $i \leftarrow 0$
\WHILE{$i < k$}
\STATE $s \leftarrow \initstate$
\STATE $q \leftarrow q_0$
\STATE $r \leftarrow 0$
\WHILE{r = 0}
\STATE Choose action $a$ according to the RL policy
\STATE Take action $a$, observe next state $s'$, and time $\tau$
\STATE Choose transition $t$ in $A$ according to the RL policy
\STATE Take transition $t$ in $A$, observe next state $q'$
\STATE $r \leftarrow R'(s,q,a)$
\STATE $Q_f(s,q,a) \leftarrow Q_f(s,q,a) +\alpha \bigl[ r + e^{-\gamma\tau} \max_{a' \in \actions} Q_f(s',q',a')- Q_f(s,q,a) \bigr]$
\STATE $s \leftarrow s'$
\STATE $q \leftarrow q'$
\ENDWHILE
\STATE $i \leftarrow i+1$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

Line 1 initialises the Q function which is defined as $Q_f: \states \times Q \times \actions \rightarrow \mathbb{R}$. Line 2 initialises $i$ which keeps the count of number of episodes completed. The algorithms conducts $k$ episodes. The variables $s$ and $q$ represents the current state of the CTMDP and SLDBW respectively and is initialised to their initial states. The action $a$ from the current state of CTMDP and the transition $t$ from the state of SLDBW is picked according to the RL policy used (eg. $\epsilon$-greedy). From the results in section \ref{sec:theorems&algo}, we define the reward function $R'$. For a given state $(s,q)$ and action $a$, $$
R'((s,q),a) = \begin{cases}
1 \text{ with probability $1-\zeta$} & \text{if (s,q) is accepting}\\
0 & \text{otherwise}
\end{cases}
$$
where $\zeta \in (0,1)$. Variable $r$ stores the reward obtained in each iteration of the episode. An episode ends when a positive reward is received, i.e, when $r > 0$. 

% \begin{algorithm}
% \caption{Algorithm for expectation semantics}\label{algo:expt}
% \hspace*{\algorithmicindent} \textbf{Input:}  \text{Initial state $s_{init}$, SLDBW $A$, discount factor $\gamma$,}\\
% \hspace*{\algorithmicindent} \hspace{11mm}\text{reward function $R'$, number of episodes $k$,} \\
% \hspace*{\algorithmicindent}\hspace{11mm} \text{learning rate $\alpha$, episode length $eplen$}\\
% \hspace*{\algorithmicindent} \textbf{Output:}  \text{Optimal strategy $\sigma$}
% \begin{algorithmic}[1]
% \STATE Initialise $Q_f$ to all zeroes
% \STATE $i \leftarrow 0$
% \WHILE{$i < k$}
% \STATE $s \leftarrow \initstate$
% \STATE $q \leftarrow q_0$
% \STATE $r \leftarrow 0$
% \STATE $j \leftarrow 0$
% \WHILE{$j < eplen$}
% \STATE Choose action $a$ according to the RL policy
% \STATE Take action $a$, observe next state $s'$, and time $\tau$
% \STATE Choose transition $t$ in SLDBW according to the RL policy
% \STATE Take transition $t$ in SLDBW, observe next state $q'$
% \STATE $r \leftarrow R'(s,q,a,\tau)$
% \STATE $Q_f(s,q,a) \leftarrow Q_f(s,q,a) +\alpha \bigl[ r + e^{-\gamma\tau} \max_{a' \in \actions} Q_f(s',q',a')- Q_f(s,q,a) \bigr]$
% \STATE $s \leftarrow s'$
% \STATE $q \leftarrow q'$
% \ENDWHILE
% \STATE $i \leftarrow i+1$
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}
%  The algorithm for expectation semantics (algorithm \ref{algo:expt}) is similar to that of satisfaction semantics, here the termination of an episode is based on the user defined variable $eplen$ and the reward function $R'$ is based on the reward function defined in section \ref{sec:d_time}. The reward function is defined as 
%  $$
%  R'((s,q),a,\tau) = \begin{cases}
%  \tau & \text{if ($s,q$) is an accepting state}\\
%  0 & \text{otherwise}
%  \end{cases}
%  $$

==> csl.tex <==
% \subsection{Limiting Distribution of a CTMC}
% Limiting distribution of a CTMC gives the probability of being in a state in the `long run' or when time is infinity at the limit. Consider a CTMC $H$ where $\states$ is the set of states and $\initstate$ is the initial state. We define a random variable $X(t)$ for $t \in \realpositives$ to be the  state at which the CTMC $H$ is in at time $t$. We define the limiting distribution of $H$ as $\pi^{H} = [\pi_{s_1}^{H}, \pi_{s_2}^H... \pi_{s_n}^H]$ where $s_1,s_2...s_n \in \states$ and for each state $s_i \in \states$
% \begin{center}
%     $\pi^H_{s_i} = \lim_{t \rightarrow \infty} P(X(t) = s_i | X(0) = \initstate)$
% \end{center}
% Also $\sum_{s_i \in S} \pi^{H}_{s_i} = 1$. We omit $X(0) = \initstate$ when the initial state is clear from the context. For a set $T$ of states, we define the limiting probability of $T$ as $\pi_{T}^{H} = \sum_{s \in T} \pi^{H}_{s}$. For a given CTMDP $\Mdp$, a pure strategy $\sigma$, and set $T$ of states, we show the relationship between the expected average reward with respect to the reward function $r'$ and the limiting probability of $T$ in the CTMC $\Mdp^{[\sigma]}$.

% \begin{lemma}\label{csl1}
% For a given CTMDP $\Mdp$, a pure strategy $\sigma$, and a set $T$ of states,
% \[
% Ear^{\Mdp^{[\sigma]}}(T) = \pi_{T}^{\Mdp^{[\sigma]}}
% \]
% where $\pi_{T}^{\Mdp^{[\sigma]}}$ is the limiting probability of $T$.
% \end{lemma}
% \begin{proof}
%  We define the expected average reward from a CTMC $\ctmc$ as,
% \begin{equation*}
%     \begin{split}
%  Ear^{\ctmc} = \lim_{n \rightarrow \infty} \frac{\mathbb{E}_{\sigma}^{\Mdp} \{\sum^{n}_{i=0} r(s_i,a_i)\}}{\mathbb{E}_{\sigma}^{\Mdp} \{\sum_{i=0}^{n} \tau_i\}}
%  \end{split}
% \end{equation*}
% From the definition of reward function r', it gives a reward of $1$ for one time unit spent in a state in $T$ and $0$ otherwise. Therefore, the expected average reward becomes,
% \[
% Ear^{\ctmc} = \lim_{n \rightarrow \infty} \frac{\mathbb{E}_{\sigma}^{\Mdp} \{\sum_{i=0,s_i \in T}^{n}\tau_{s_{i}}\}}{\mathbb{E}_{\sigma}^{\Mdp} \{\sum_{i=0}^{n} \tau_i\}}
% \]
% where $\sum_{i=0,s_i \in T}^{n}\tau_{s_{i}}$ gives the expected time spent in states of $T$ and $\sum_{i=0}^{n} \tau_i$ is the total time. This gives the fraction of time spent in states of $T$ in the long run (i.e when $t \rightarrow \infty$) i.e,
% \[
% \sum_{s_i \in T}\lim_{t \rightarrow \infty} P(X(t) = s_i) = \lim_{n \rightarrow \infty} \frac{\mathbb{E}_{\sigma}^{\Mdp} \{\sum_{i=0,s_i \in T}^{n}\tau_{s_{i}}\}}{\mathbb{E}_{\sigma}^{\Mdp} \{\sum_{i=0}^{n} \tau_i\}}
% \]
 
%  From the definition of $\pi_{T}^{\Mdp^{[\sigma]}}$, we can conclude that 
% \[
% Ear^{\ctmc} = \pi_{T}^{\ctmc}
% \]
% \end{proof}
% From Lemma \ref{csl1}, it is clear that for a given set $T$ of states, a reward function $r'$, and a strategy $\sigma$, the expected average reward and the limiting probability of $T$ in the resulting CTMC are the same.

% \begin{theorem}\label{csl2}
% For a CTMDP $M$, and a set $T$ of states, an optimal pure strategy $\sigma^*$ maximising the expected average reward with respect to $r'$ results in a CTMC $M^{[\sigma^*]}$ which also maximises the limiting probability of $T$.
% \end{theorem}
% \begin{proof}
% From Lemma \ref{csl1}, for each pure strategy $\sigma$,
% \[
% Ear^{\Mdp^{[\sigma]}}(T) = \pi_{T}^{\Mdp^{[\sigma]}}
% \]
% Therefore, if $\sigma^*$ is the strategy maximising the expected average reward then we can conclude that it also maximises the limiting probability of $T$.
% \end{proof}
% From Theorem \ref{csl2}, it is clear that the reward function $r'$ gives the optimal pure strategy that maximises the limiting probability of $T$. From Theorem \ref{csl2}, and  Corollary \ref{corollary:1}, we obtain the following.
% \begin{corollary}\label{corollary2}
% For a CTMDP $\Mdp$, a set $T$ of states and a reward function $r'$, there exists a Blackwell optimal pure strategy $\sigma^*$ such that it maximises \begin{inparaenum}
% \item the expected average reward, 
% \item and the limiting probability of $T$ is maximised in $\Mdp^{[\sigma^*]}$.
% \end{inparaenum}
% \end{corollary}
% From Corollary \ref{corollary2}, it is clear that given a set $T$ of states, the problem of obtaining an optimal strategy maximising the expected average reward and obtaining a strategy which maximises the limiting probability of $T$ are the same.

% Finally, we describe the relation between continuous time stochastic logic(CSL) \cite{baier1999CSL} which is a stochastic branching time temporal logic that is used to model-check CTMCs against properties expressed in it and our expectation semantics.
% This logic contains a steady state operator $\mathcal{S}$ and maximizing the probability of satisfaction of this $\mathcal{S}$ for a formula that is true in the good states of a CTMDP corresponds to maximising the expected time of stay in these sttaes.

\begin{comment}
{\color{red} What did we decide regarding CSLs?}
Continuous time stochastic logic(CSL) \cite{baier1999CSL} is a stochastic branching time temporal logic and is used to model-check CTMCs against properties expressed in it. We show the relationship between expectation semantics and CSL.
\subsection{CSL}
Consider a CTMC $H$, the state formulas of CSL are interpreted over the states of $H$. Let $a \in \atomicprop$, and $p \in [0,1]$, the syntax of a state formula is defined by:
\begin{center}
    $\phi := True | a | \phi_1 \land \phi_2 | \lnot \phi | \mathcal{S}_{\bowtie p}(\phi) | \mathcal{P}_{\bowtie p}(\psi)$
\end{center}
Let $I \subseteq \realpositives $ be an interval. A path formula is defined by:
\begin{center}
    $\psi := \nextt \phi | \phi_1 \until \phi_2 | \phi_1 \until^{I} \phi_2$
\end{center}
Where $\bowtie \in \{\geq,\leq\}$.
Here the meaning of $\nextt$ and $\until$ is the same as LTL. The operator $\until^I$ is a timed variant of until operator used in LTL. For a path $\rho$ in a CTMC, we denote the state of $\rho$ at time $t$ by $\rho[t]$. For a time interval $I$, a formula $\phi_1 \until^I \phi_2$ is satisfied if there exists a path $\rho$ such that there exists a time $t \in I$ where $\rho[t]$ satisfies $\phi_2$ and for all $u \in [0,t)$ $\rho[u]$ satisfies $\phi_1$. The operator $\mathcal{S}_{\bowtie p}(\phi)$ is satisfied if the limiting probability of $sat (\phi)$ (the set of states satisfying $\phi$) is $q$ and $q\bowtie p$. The operator $\mathcal{P}_{\bowtie p}(\phi)$ is satisfied if the probability of paths from a state s satisfying $\phi$ is $q$ and $q\bowtie p$. We concentrate on the $S$ operator and relate it to the expectation semantics.

The semantics of state and path formulas are the same as that of LTL, and we denote the semantics of $\mathcal{S}$ operator as
\begin{center}
    $\initstate \models \mathcal{S}_{\bowtie p}(\phi)$ iff $\pi^{H}_{Sat(\phi)} \bowtie p$,
\end{center}
where $sat(\phi)$ is the set of states satisfying the formula $\phi$. 

For a CTMDP $\Mdp$, we say that it satisfies a CSL formula $\phi$ if there exists a strategy $\sigma$ such that $\Mdp^{[\sigma]}$ satisfies $\phi$. We look at formulas of the form $\mathcal{S}_{\geq p}(\phi)$ that are called steady-state formulas, where $\phi$ is an LTL formula. We show that the reward function $r'$ can be used to check if there exists a strategy that satisfies a steady-state formula. We provide a sketch of this procedure.


Given an $\omega$-regular property $\phi$, Theorem \ref{GFM} states that a corresponding \textbf{GFM} $A_\phi$ exists. For a given CTMDP $M$ and a \textbf{GFM} $A_\phi$, let $(\Mdp \times A_\phi)$ be the product CTMDP as defined in Section~\ref{prelims}. Let $Acc$ be the set of accepting states in $(\Mdp \times \caut)$. We can construct a reward function $r'$ with respect to $Acc$ as shown previously. From Theorem~\ref{csl2}, a strategy maximising the expected average reward also maximises the limiting probability for $Acc$. Let $\sigma^*$ be an optimal pure strategy in $(\Mdp \times \caut)$ maximising the expected average reward. Therefore, $\sigma^*$ also maximises the limiting probability for the states in $Acc$ in $(\Mdp \times A_{\phi})^{[\sigma^*]}$ and let this limiting probability be denoted by $q_{Acc}$, i.e, 
\begin{center}
$q_{Acc} = \sum_{s \in Acc} \pi^{(\Mdp \times A_{\phi})^{[\sigma^*]}}_{s}(\phi)$    
\end{center}


From the semantics of CSL, a formula $\mathcal{S}_{\geq p}  (\phi)$ is satisfied in $(\Mdp \times \caut)$ if there exists a strategy $\sigma$ such that 
\begin{center}
    $\pi^{(\Mdp \times \caut)^{[\sigma]}}_{sat(\phi)} \geq p$
\end{center}
From the definitions, we know that $sat(\phi) = Acc$ and as $\sigma^*$ is an optimal pure strategy maximising the limiting probability of $Acc$, we can conclude that $(\Mdp \times A_\phi)$ satisfies $\mathcal{S}_{\geq p}(\phi)$ iff $q_{Acc} \geq p$.
\end{comment}






==> reward_machines.tex <==
In the classical RL literature, the learning objective is specified using
Markovian reward functions, i.e. a function $\rho: S \times A \to \Real$
assigning utility to state-action pairs. 
A {\it rewardful} MDP is a tuple $\Mm = (S, s_0, A, T, \rho)$ where $S, s_0, A,$ and $T$ are defined in a similar way as for MDPa, and $\rho$ is a Markovian reward function.
%, where $\Mm$ is an MDP
%and $\rho\colon S \times A \to \Real$ is a reward function 
A rewardful MDP $\Mm$ under a
strategy $\sigma$ determines a sequence of random rewards
${\rho(X_{i-1}, Y_i)}_{i \geq 1}$, where $X_i$ and $Y_i$ are the
random variables denoting the $i$-th state and action, respectively.
%% The {\it reachability probability} objective $\PReach(T)^\Mm_\sigma(s)$ (with
%% $T \subseteq S$) is defined as
%% $\Pr^\Mm_\sigma(s) \set{\seq{s,a_1,s_1,\ldots} \in \Runs_\sigma^\Mm(s)
%%   \colon \exists i \scope s_i \in T}$.
  For
$\lambda \in [0, 1[$, the {\it discounted reward} 
$\EDisct(\lambda)^\Mm_\sigma(s)$ is defined as
\[
\lim_{N \to \infty} \eE^\Mm_\sigma(s) \set{\sum_{1 \leq i \leq N}
  \lambda^{i-1} \rho(X_{i-1}, Y_i)},
\]
while the {\it average
  reward} $\EAvg^\Mm_\sigma(s)$ is defined as
\[
\limsup_{N \to \infty} \frac{1}{N} \eE^\Mm_\sigma(s)\set{\sum_{1\leq i \leq
    N} \rho(X_{i-1}, Y_i)}.
\]
For an objective $\ECost^\Mm {\in} \{\EDisct(\lambda)^\Mm,
\EAvg^\Mm\}$ and state $s$, we define the optimal reward
$\ECost^\Mm_*(s)$ as $\sup_{\sigma \in \Strat_\Mm} \ECost^\Mm_\sigma(s)$.  
A strategy $\sigma$ is optimal for $\ECost^\Mm$ if
$\ECost^\Mm_\sigma(s) {=} \ECost^\Mm_*(s)$ for all $s {\in} S$.
The optimal cost and strategies for these objectives can be computed in
polynomial time~\cite{Puterman94}.  

Often, complex learning objectives cannot be expressed using Markovian reward
signals. 
A recent trend is to express learning objectives using finite-state reward
machines~\cite{icarte2018using}. 
We require a more expressive variant of reward machine capable of $\epsilon$ transitions and nondeterminisim. We
call them nondeterministic reward machines. 
A (nondeterministic) reward machine is a tuple $\Rr = (\Sigma_\epsilon, U, u_0, \delta_r, \rho)$
where $U$ is a finite set of states, $u_0 \in U$ is the starting state,
$\delta_r: U \times \Sigma_\epsilon \to 2^U$ is the transition relation, 
and $\rho: U \times \Sigma_\epsilon \times U \to \Real$ is the reward function, where $\Sigma_\epsilon = (\Sigma\cup \set{\epsilon})$ and $\epsilon$ is a special silent transition.

Given an MDP $\Mm = (S, s_0, A, T, AP, L)$ and a reward machine $\Rr = (\Sigma_\epsilon, U, u_0, \delta_r, \rho)$ over the alphabet $\Sigma = 2^{AP}$,  their product 
\[
\Mm\times\Rr = (S{\times} U, s_0 {\times} u_0, (A {\times} U) \cup\set{\epsilon},
T^\times, \rho^\times)
\]
is a rewardful MDP where
$T^\times: (S {\times} U) \times ((A {\times} U) \cup \set{\epsilon}) \to \DIST(S{\times} U)$ is such that
$T^\times((s,u), \alpha)(({s}',{u}'))$ equals 
\begin{multline*}
%T^\times((s,u), \alpha)(({s}',{u}')) =\\
\begin{cases}
T(s,a)({s}') & \text{if } \alpha = (a, u') \text{ and } (u,L(s),u') \in \delta_r \\
1 & \text{if } \alpha = \epsilon \text{ and } s = s' \text{ and } \delta(u, \epsilon, {u}') \in \delta_r \\
0 & \text{otherwise.}
\end{cases}
\end{multline*}
and $\rho^\times: (S{\times} U) \times ((A {\times}
U) \cup \set{\epsilon}) \times (S{\times} U)\to \Real$ is defined such that 
$\rho^\times((s,u), \alpha, (s', u'))$ equals
\begin{multline*}
% \rho^\times((s,u), \alpha, (s', u')) =\\
\begin{cases}
\rho(u, L(s), u') & \text{if } \alpha = (a, u') \text{ and } (u,L(s),{u}') \in \delta_r \\
\rho(u, \epsilon, u') & \text{if } \alpha = \epsilon.
\end{cases}
\end{multline*}
For technical convenience, we assume that $\Mm{\times}\Rr$ contains only reachable states from $(s_0, u_0)$.
For both discounted and average objectives, the optimal strategies of
$\Mm{\times}\Rr$ are positional on $\Mm{\times}\Rr$.
Moreover, these positional strategies characterize a finite memory strategy (with memory skeleton based on the  states of $\Rr$ and the next-action function based on the positional strategy) over $\Mm$
maximizing the learning objective given by $\Rr$. 

